Privacy Budget Scheduling

Machine learning (ML) models trained on personal data have been shown to leak information about users. Differential privacy (DP) enables model training with a guaranteed bound on this leakage. Each new model trained with DP increases the bound on data leakage and can be seen as consuming part of a global privacy budget that should not be exceeded. This budget is a scarce resource that must be carefully managed to maximize the number of successfully trained models. We describe PrivateKube, an extension to the popular Kubernetes datacenter orchestrator that adds privacy as a new type of resource to be managed alongside other traditional compute resources, such as CPU, GPU, and memory. The abstractions we design for the privacy resource mirror those defined by Kubernetes for traditional resources, but there are also major differences. For example, traditional compute resources are replenishable while privacy is not: a CPU can be regained after a model finishes execution while privacy budget cannot. This distinction forces a re-design of the scheduler. We present DPF (Dominant Private Block Fairness) -- a variant of the popular Dominant Resource Fairness (DRF) algorithm -- that is geared toward the non-replenishable privacy resource but enjoys similar theoretical properties as DRF. We evaluate PrivateKube and DPF on microbenchmarks and an ML workload on Amazon Reviews data. Compared to existing baselines, DPF allows training more models under the same global privacy guarantee. This is especially true for DPF over R\'enyi DP, a highly composable form of DP.

==> Makefile <==
PAPER=paper
LATEX=pdflatex

BIBTEX=bibtex

SRCS=$(PAPER).tex $(wildcard sections/*.tex)
REFS=$(wildcard bib/*.bib)
FIGS=$(wildcard figures/*)
STYLE=$(wildcard style/*)

.PHONY: results $(PAPER).pdf clean

all: results $(PAPER).pdf

results:
	+make -C $@

$(PAPER).pdf: $(SRCS) $(REFS) $(FIGS) $(STYLE)
	$(LATEX) $(PAPER)
	$(BIBTEX) $(PAPER)
	$(LATEX) $(PAPER)
	$(LATEX) $(PAPER)

submission: $(PAPER).pdf
	cp $(PAPER).pdf submission/

clean:
	rm -f *.dvi *.aux *.log *.blg *.bbl \
          $(PAPER).ps $(PAPER).pdf \
          $(PAPER)-single.pdf $(PAPER)-single.ps
	(cd results; make clean)


==> appendices/remaining-evaluation.tex <==
% See artifact.tex instead


==> appendices/scheduling-algos-for-presentations.tex <==
\setcounter{algorithm}{0}

\begin{algorithm}[!t]
    \caption{{\bf DRF} (max-min fairness over $m$ resources).}
    \begin{algorithmic}
        \State {\color{gray} \# $R = <R_1,...,R_m>$ resource capacities;}
        \State {\color{gray} \# $C = <C_1,...,C_m>$ consumed resources.}
        \Function{DominantShare}{demand vector $d_i$}
        \State return $\max_j \ \frac{d_{i,j}}{R_j}$
        \EndFunction
        \Function{onSchedulerTimer}{waiting jobs w}
        \State $\textrm{sorted\_jobs} \gets$ sortBy(\textproc{DominantShare}, w)
        \For{$i$ in  $\textrm{sorted\_jobs}$}
        \If{$C+d_i \le R$}
        \State $C=C+d_i$
        \EndIf
        \EndFor
        \EndFunction
    \end{algorithmic}
    \label{alg:drf-ppt}
\end{algorithm}



\begin{algorithm}[!t]
    \caption{{\bf DPF-N} (max-min fairness for first $N$ pipelines over $m$ private blocks).}
    \begin{algorithmic}
        \State {\color{gray} \# $R = <\epsilon^G_1,...,\epsilon^G_m>$ private blocks capacities;}
        \State {\color{gray} \# $U = <\epsilon^U_1,...,\epsilon^U_m>$ unlocked budgets.}
        \State {\color{gray} \# $C = <\epsilon^C_1,...,\epsilon^C_m>$ consumed budgets.}
        \Function{onBlockCreation}{private block $j$}
        \State $U_j\gets 0$
        \EndFunction
        \Function{onPipelineArrival}{demand vector $d_{i}$}
        \For{$\forall j: d_{i,j}>0$}
        \State $U_j \gets \min(R_j, \ U_j + \frac{R_j}{N})$
        \EndFor
        \EndFunction
        \Function{DominantShare}{demand vector $d_i$}
        \State return $\max_j \ \frac{d_{i,j}}{R_j}$
        \EndFunction
        \Function{onSchedulerTimer}{waiting pipelines w}
        \State {\color{gray} \# Similar to DRF, except ``if'' condition is: $C+d_i \le U$.}
        \EndFunction
    \end{algorithmic}
    \label{alg:dpf-ppt}
\end{algorithm}


==> results/Makefile <==
FIGS = place_holder

GNUPLOT := gnuplot
EPS2PDF := epstopdf
EPS2PNG := convert
PDFFILES = $(FIGS:=.pdf)
PNGFILES = $(FIGS:=.png)

all: $(PDFFILES) Makefile
	$(MAKE) -C simulator
	$(MAKE) -C individual_models/others
	$(MAKE) -C individual_models/all-product
	$(MAKE) -C individual_models/product-lstm
	$(MAKE) -C evaluation/allocation_fraction
	$(MAKE) -C evaluation/delay_cdf
	$(MAKE) -C evaluation/job_sizes
	$(MAKE) -C evaluation/workload-mix/product
	$(MAKE) -C evaluation/workload-mix/sentiment
	$(MAKE) -C evaluation/workload-mix/stats


pngs: $(PNGFILES)

list:
	@echo $(PDFFILES) $(PNGFILES)

%.pdf: %.eps
	$(EPS2PDF) $< --outfile $@.tmp.pdf
	gs -dCompatibilityLevel=1.4 -dPDFSETTINGS=/screen -dCompressFonts=true -dSubsetFonts=true -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sOutputFile=$@ -c ".setpdfwrite <</NeverEmbed [ ]>> setdistillerparams" -f $@.tmp.pdf
	rm $@.tmp.pdf

%.png: %.eps
	$(EPS2PNG) $< -background white -alpha remove -alpha off -rotate 90 $@

%.eps: %.plot %.dat boilerplate* Makefile
	$(GNUPLOT) -e "set terminal post monochrome; set output \"$@\"" $<

clean:
	$(MAKE) -C simulator clean
	$(MAKE) -C individual_models/others clean
	$(MAKE) -C individual_models/all-product clean
	$(MAKE) -C individual_models/product-lstm clean
	$(MAKE) -C evaluation/allocation_fraction clean
	$(MAKE) -C evaluation/delay_cdf clean
	$(MAKE) -C evaluation/job_sizes clean
	$(MAKE) -C evaluation/workload-mix/product clean
	$(MAKE) -C evaluation/workload-mix/sentiment clean
	$(MAKE) -C evaluation/workload-mix/stats clean


==> results/evaluation/allocation_fraction/Makefile <==
FIGS = allocation_fraction_old allocation_fraction_rdp allocation_fraction_nordp

GNUPLOT := gnuplot
EPS2PDF := epstopdf
EPS2PNG := convert
PDFFILES = $(FIGS:=.pdf)
PNGFILES = $(FIGS:=.png)

all: $(PDFFILES) Makefile

pngs: $(PNGFILES)

list:
	@echo $(PDFFILES) $(PNGFILES)

%.pdf: %.eps
	$(EPS2PDF) $< --outfile $@.tmp.pdf
	gs -dCompatibilityLevel=1.4 -dPDFSETTINGS=/screen -dCompressFonts=true -dSubsetFonts=true -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sOutputFile=$@ -c ".setpdfwrite <</NeverEmbed [ ]>> setdistillerparams" -f $@.tmp.pdf
	rm $@.tmp.pdf

%.png: %.eps
	$(EPS2PNG) $< -background white -alpha remove -alpha off -rotate 90 $@

%.eps: %.plot %.csv boilerplate* Makefile
	$(GNUPLOT) -e "set terminal post monochrome; set output \"$@\"" $<

clean:
	@rm -f $(PDFFILES)


==> results/evaluation/delay_cdf/Makefile <==
FIGS = cdf_old cdf_rdp cdf_nordp

GNUPLOT := gnuplot
EPS2PDF := epstopdf
EPS2PNG := convert
PDFFILES = $(FIGS:=.pdf)
PNGFILES = $(FIGS:=.png)

all: $(PDFFILES) Makefile

pngs: $(PNGFILES)

list:
	@echo $(PDFFILES) $(PNGFILES)

%.pdf: %.eps
	$(EPS2PDF) $< --outfile $@.tmp.pdf
	gs -dCompatibilityLevel=1.4 -dPDFSETTINGS=/screen -dCompressFonts=true -dSubsetFonts=true -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sOutputFile=$@ -c ".setpdfwrite <</NeverEmbed [ ]>> setdistillerparams" -f $@.tmp.pdf
	rm $@.tmp.pdf

%.png: %.eps
	$(EPS2PNG) $< -background white -alpha remove -alpha off -rotate 90 $@

%.eps: %.plot boilerplate* Makefile
	$(GNUPLOT) -e "set terminal post monochrome; set output \"$@\"" $<

clean:
	@rm -f $(PDFFILES)


==> results/evaluation/job_sizes/Makefile <==
FIGS = N400_event incoming

GNUPLOT := gnuplot
EPS2PDF := epstopdf
EPS2PNG := convert
PDFFILES = $(FIGS:=.pdf)
PNGFILES = $(FIGS:=.png)

all: $(PDFFILES) Makefile

pngs: $(PNGFILES)

list:
	@echo $(PDFFILES) $(PNGFILES)

%.pdf: %.eps
	$(EPS2PDF) $< --outfile $@.tmp.pdf
	gs -dCompatibilityLevel=1.4 -dPDFSETTINGS=/screen -dCompressFonts=true -dSubsetFonts=true -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sOutputFile=$@ -c ".setpdfwrite <</NeverEmbed [ ]>> setdistillerparams" -f $@.tmp.pdf
	rm $@.tmp.pdf

%.png: %.eps
	$(EPS2PNG) $< -background white -alpha remove -alpha off -rotate 90 $@

%.eps: %.plot boilerplate* Makefile
	$(GNUPLOT) -e "set terminal post monochrome; set output \"$@\"" $<

clean:
	@rm -f $(PDFFILES)


==> results/evaluation/workload-mix/all/Makefile <==
FIGS = workload-mix

GNUPLOT := gnuplot
EPS2PDF := epstopdf
EPS2PNG := convert
PDFFILES = $(FIGS:=.pdf)
PNGFILES = $(FIGS:=.png)

all: $(PDFFILES) Makefile

pngs: $(PNGFILES)

list:
	@echo $(PDFFILES) $(PNGFILES)

%.pdf: %.eps
	$(EPS2PDF) $< --outfile $@.tmp.pdf
	gs -dCompatibilityLevel=1.4 -dPDFSETTINGS=/screen -dCompressFonts=true -dSubsetFonts=true -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sOutputFile=$@ -c ".setpdfwrite <</NeverEmbed [ ]>> setdistillerparams" -f $@.tmp.pdf
	rm $@.tmp.pdf

%.png: %.eps
	$(EPS2PNG) $< -background white -alpha remove -alpha off -rotate 90 $@

%.eps: %.plot %.csv boilerplate* Makefile
	$(GNUPLOT) -e "set terminal post monochrome; set output \"$@\"" $<

clean:
	@rm -f $(PDFFILES)


==> results/evaluation/workload-mix/product/Makefile <==
FIGS = workload-mix

GNUPLOT := gnuplot
EPS2PDF := epstopdf
EPS2PNG := convert
PDFFILES = $(FIGS:=.pdf)
PNGFILES = $(FIGS:=.png)

all: $(PDFFILES) Makefile

pngs: $(PNGFILES)

list:
	@echo $(PDFFILES) $(PNGFILES)

%.pdf: %.eps
	$(EPS2PDF) $< --outfile $@.tmp.pdf
	gs -dCompatibilityLevel=1.4 -dPDFSETTINGS=/screen -dCompressFonts=true -dSubsetFonts=true -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sOutputFile=$@ -c ".setpdfwrite <</NeverEmbed [ ]>> setdistillerparams" -f $@.tmp.pdf
	rm $@.tmp.pdf

%.png: %.eps
	$(EPS2PNG) $< -background white -alpha remove -alpha off -rotate 90 $@

%.eps: %.plot %.csv boilerplate* Makefile
	$(GNUPLOT) -e "set terminal post monochrome; set output \"$@\"" $<

clean:
	@rm -f $(PDFFILES)


==> results/evaluation/workload-mix/sentiment/Makefile <==
FIGS = workload-mix

GNUPLOT := gnuplot
EPS2PDF := epstopdf
EPS2PNG := convert
PDFFILES = $(FIGS:=.pdf)
PNGFILES = $(FIGS:=.png)

all: $(PDFFILES) Makefile

pngs: $(PNGFILES)

list:
	@echo $(PDFFILES) $(PNGFILES)

%.pdf: %.eps
	$(EPS2PDF) $< --outfile $@.tmp.pdf
	gs -dCompatibilityLevel=1.4 -dPDFSETTINGS=/screen -dCompressFonts=true -dSubsetFonts=true -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sOutputFile=$@ -c ".setpdfwrite <</NeverEmbed [ ]>> setdistillerparams" -f $@.tmp.pdf
	rm $@.tmp.pdf

%.png: %.eps
	$(EPS2PNG) $< -background white -alpha remove -alpha off -rotate 90 $@

%.eps: %.plot %.csv boilerplate* Makefile
	$(GNUPLOT) -e "set terminal post monochrome; set output \"$@\"" $<

clean:
	@rm -f $(PDFFILES)


==> results/evaluation/workload-mix/stats/Makefile <==
FIGS = workload-mix

GNUPLOT := gnuplot
EPS2PDF := epstopdf
EPS2PNG := convert
PDFFILES = $(FIGS:=.pdf)
PNGFILES = $(FIGS:=.png)

all: $(PDFFILES) Makefile

pngs: $(PNGFILES)

list:
	@echo $(PDFFILES) $(PNGFILES)

%.pdf: %.eps
	$(EPS2PDF) $< --outfile $@.tmp.pdf
	gs -dCompatibilityLevel=1.4 -dPDFSETTINGS=/screen -dCompressFonts=true -dSubsetFonts=true -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sOutputFile=$@ -c ".setpdfwrite <</NeverEmbed [ ]>> setdistillerparams" -f $@.tmp.pdf
	rm $@.tmp.pdf

%.png: %.eps
	$(EPS2PNG) $< -background white -alpha remove -alpha off -rotate 90 $@

%.eps: %.plot %.csv boilerplate* Makefile
	$(GNUPLOT) -e "set terminal post monochrome; set output \"$@\"" $<

clean:
	@rm -f $(PDFFILES)


==> results/individual_models/all-product/Makefile <==
FIGS = all-product

GNUPLOT := gnuplot
EPS2PDF := epstopdf
EPS2PNG := convert
PDFFILES = $(FIGS:=.pdf)
PNGFILES = $(FIGS:=.png)

all: $(PDFFILES) Makefile

pngs: $(PNGFILES)

list:
	@echo $(PDFFILES) $(PNGFILES)

%.pdf: %.eps
	$(EPS2PDF) $< --outfile $@.tmp.pdf
	gs -dCompatibilityLevel=1.4 -dPDFSETTINGS=/screen -dCompressFonts=true -dSubsetFonts=true -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sOutputFile=$@ -c ".setpdfwrite <</NeverEmbed [ ]>> setdistillerparams" -f $@.tmp.pdf
	rm $@.tmp.pdf

%.png: %.eps
	$(EPS2PNG) $< -background white -alpha remove -alpha off -rotate 90 $@

%.eps: %.plot %.csv Makefile
	$(GNUPLOT) -e "set terminal post monochrome; set output \"$@\"" $<

clean:
	@rm -f $(PDFFILES)


==> results/individual_models/others/Makefile <==
FIGS = product-bow-event product-bow-user-time product-bow-user

GNUPLOT := gnuplot
EPS2PDF := epstopdf
EPS2PNG := convert
PDFFILES = $(FIGS:=.pdf)
PNGFILES = $(FIGS:=.png)

all: $(PDFFILES) Makefile

pngs: $(PNGFILES)

list:
	@echo $(PDFFILES) $(PNGFILES)

%.pdf: %.eps
	$(EPS2PDF) $< --outfile $@.tmp.pdf
	gs -dCompatibilityLevel=1.4 -dPDFSETTINGS=/screen -dCompressFonts=true -dSubsetFonts=true -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sOutputFile=$@ -c ".setpdfwrite <</NeverEmbed [ ]>> setdistillerparams" -f $@.tmp.pdf
	rm $@.tmp.pdf

%.png: %.eps
	$(EPS2PNG) $< -background white -alpha remove -alpha off -rotate 90 $@

%.eps: %.plot %.csv Makefile
	$(GNUPLOT) -e "set terminal post monochrome; set output \"$@\"" $<

clean:
	@rm -f $(PDFFILES)


==> results/individual_models/product-lstm/Makefile <==
FIGS = product-lstm-event product-lstm-user-time product-lstm-user

GNUPLOT := gnuplot
EPS2PDF := epstopdf
EPS2PNG := convert
PDFFILES = $(FIGS:=.pdf)
PNGFILES = $(FIGS:=.png)

all: $(PDFFILES) Makefile

pngs: $(PNGFILES)

list:
	@echo $(PDFFILES) $(PNGFILES)

%.pdf: %.eps
	$(EPS2PDF) $< --outfile $@.tmp.pdf
	gs -dCompatibilityLevel=1.4 -dPDFSETTINGS=/screen -dCompressFonts=true -dSubsetFonts=true -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sOutputFile=$@ -c ".setpdfwrite <</NeverEmbed [ ]>> setdistillerparams" -f $@.tmp.pdf
	rm $@.tmp.pdf

%.png: %.eps
	$(EPS2PNG) $< -background white -alpha remove -alpha off -rotate 90 $@

%.eps: %.plot %.csv Makefile
	$(GNUPLOT) -e "set terminal post monochrome; set output \"$@\"" $<

clean:
	@rm -f $(PDFFILES)


==> results/sage-sample-graph/Makefile <==
FIGS = end_to_end

GNUPLOT := gnuplot
EPS2PDF := epstopdf
EPS2PNG := convert
PDFFILES = $(FIGS:=.pdf)
PNGFILES = $(FIGS:=.png)

all: $(PDFFILES) Makefile

pngs: $(PNGFILES)

list:
	@echo $(PDFFILES) $(PNGFILES)

%.pdf: %.eps
	$(EPS2PDF) $< --outfile $@.tmp.pdf
	gs -dCompatibilityLevel=1.4 -dPDFSETTINGS=/screen -dCompressFonts=true -dSubsetFonts=true -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sOutputFile=$@ -c ".setpdfwrite <</NeverEmbed [ ]>> setdistillerparams" -f $@.tmp.pdf
	rm $@.tmp.pdf

%.png: %.eps
	$(EPS2PNG) $< -background white -alpha remove -alpha off -rotate 90 $@

%.eps: %.plot %.dat boilerplate* Makefile
	$(GNUPLOT) -e "set terminal post monochrome; set output \"$@\"" $<

clean:
	@rm -f $(PDFFILES)


==> results/simulator/Makefile <==
FIGS = dp_single_block_ppl_nr__N \
	dp_single_block_sched_delay_cdf__N \
	dp_single_block_ppl_nr__mice_pct \
	dp_single_block_dpf_delay_cdf__mice_pct \
	dp_multi_block_ppl_nr__N \
	dp_multi_block_sched_delay_cdf__N \
	dp_multi_block_ppl_nr__dpfnt \
	dp_multi_block_sched_delay_cdf__dpfnt \
	rdp_multi_block_ppl_nr__N \
	rdp_multi_block_sched_delay_cdf \
	rdp_single_block_ppl_nr__N \
	rdp_single_block_sched_delay_cdf__N \
	rdp_single_block_ppl_nr__mice_pct \
	rdp_single_block_dpf_delay_cdf__mice_pct \
	rdp_multi_block_ppl_nr__dpfnt \
	rdp_multi_block_sched_delay_cdf__dpfnt
	

GNUPLOT := gnuplot
EPS2PDF := epstopdf
EPS2PNG := convert
PDFFILES = $(FIGS:=.pdf)
PNGFILES = $(FIGS:=.png)

all: $(PDFFILES) Makefile

pngs: $(PNGFILES)

list:
	@echo $(PDFFILES) $(PNGFILES)

%.pdf: %.eps
	$(EPS2PDF) $< --outfile $@.tmp.pdf
	gs -dCompatibilityLevel=1.4 -dPDFSETTINGS=/screen -dCompressFonts=true -dSubsetFonts=true -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sOutputFile=$@ -c ".setpdfwrite <</NeverEmbed [ ]>> setdistillerparams" -f $@.tmp.pdf
	rm $@.tmp.pdf

%.png: %.eps
	$(EPS2PNG) $< -background white -alpha remove -alpha off -rotate 90 $@

%.eps: %.plot %.csv boilerplate* Makefile
	$(GNUPLOT) -e "set terminal post monochrome; set output \"$@\"" $<

clean:
	@rm -f $(PDFFILES)


==> results/tao-graph-1-2/Makefile <==
FIGS = end_to_end

GNUPLOT := gnuplot
EPS2PDF := epstopdf
EPS2PNG := convert
PDFFILES = $(FIGS:=.pdf)
PNGFILES = $(FIGS:=.png)

all: $(PDFFILES) Makefile

pngs: $(PNGFILES)

list:
	@echo $(PDFFILES) $(PNGFILES)

%.pdf: %.eps
	$(EPS2PDF) $< --outfile $@.tmp.pdf
	gs -dCompatibilityLevel=1.4 -dPDFSETTINGS=/screen -dCompressFonts=true -dSubsetFonts=true -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sOutputFile=$@ -c ".setpdfwrite <</NeverEmbed [ ]>> setdistillerparams" -f $@.tmp.pdf
	rm $@.tmp.pdf

%.png: %.eps
	$(EPS2PNG) $< -background white -alpha remove -alpha off -rotate 90 $@

%.eps: %.plot %.csv boilerplate* Makefile
	$(GNUPLOT) -e "set terminal post monochrome; set output \"$@\"" $<

clean:
	@rm -f $(PDFFILES)


==> results/tao-graph-1/Makefile <==
FIGS = end_to_end

GNUPLOT := gnuplot
EPS2PDF := epstopdf
EPS2PNG := convert
PDFFILES = $(FIGS:=.pdf)
PNGFILES = $(FIGS:=.png)

all: $(PDFFILES) Makefile

pngs: $(PNGFILES)

list:
	@echo $(PDFFILES) $(PNGFILES)

%.pdf: %.eps
	$(EPS2PDF) $< --outfile $@.tmp.pdf
	gs -dCompatibilityLevel=1.4 -dPDFSETTINGS=/screen -dCompressFonts=true -dSubsetFonts=true -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sOutputFile=$@ -c ".setpdfwrite <</NeverEmbed [ ]>> setdistillerparams" -f $@.tmp.pdf
	rm $@.tmp.pdf

%.png: %.eps
	$(EPS2PNG) $< -background white -alpha remove -alpha off -rotate 90 $@

%.eps: %.plot %.csv boilerplate* Makefile
	$(GNUPLOT) -e "set terminal post monochrome; set output \"$@\"" $<

clean:
	@rm -f $(PDFFILES)


==> results/tao-graph-2-2/Makefile <==
FIGS = dpf

GNUPLOT := gnuplot
EPS2PDF := epstopdf
EPS2PNG := convert
PDFFILES = $(FIGS:=.pdf)
PNGFILES = $(FIGS:=.png)

all: $(PDFFILES) Makefile

pngs: $(PNGFILES)

list:
	@echo $(PDFFILES) $(PNGFILES)

%.pdf: %.eps
	$(EPS2PDF) $< --outfile $@.tmp.pdf
	gs -dCompatibilityLevel=1.4 -dPDFSETTINGS=/screen -dCompressFonts=true -dSubsetFonts=true -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sOutputFile=$@ -c ".setpdfwrite <</NeverEmbed [ ]>> setdistillerparams" -f $@.tmp.pdf
	rm $@.tmp.pdf

%.png: %.eps
	$(EPS2PNG) $< -background white -alpha remove -alpha off -rotate 90 $@

%.eps: %.plot %.csv boilerplate* Makefile
	$(GNUPLOT) -e "set terminal post monochrome; set output \"$@\"" $<

clean:
	@rm -f $(PDFFILES)


==> results/tao-graph-2/Makefile <==
FIGS = dpf

GNUPLOT := gnuplot
EPS2PDF := epstopdf
EPS2PNG := convert
PDFFILES = $(FIGS:=.pdf)
PNGFILES = $(FIGS:=.png)

all: $(PDFFILES) Makefile

pngs: $(PNGFILES)

list:
	@echo $(PDFFILES) $(PNGFILES)

%.pdf: %.eps
	$(EPS2PDF) $< --outfile $@.tmp.pdf
	gs -dCompatibilityLevel=1.4 -dPDFSETTINGS=/screen -dCompressFonts=true -dSubsetFonts=true -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sOutputFile=$@ -c ".setpdfwrite <</NeverEmbed [ ]>> setdistillerparams" -f $@.tmp.pdf
	rm $@.tmp.pdf

%.png: %.eps
	$(EPS2PNG) $< -background white -alpha remove -alpha off -rotate 90 $@

%.eps: %.plot %.csv boilerplate* Makefile
	$(GNUPLOT) -e "set terminal post monochrome; set output \"$@\"" $<

clean:
	@rm -f $(PDFFILES)


==> results/tao-graph-3-2/Makefile <==
FIGS = end_to_end

GNUPLOT := gnuplot
EPS2PDF := epstopdf
EPS2PNG := convert
PDFFILES = $(FIGS:=.pdf)
PNGFILES = $(FIGS:=.png)

all: $(PDFFILES) Makefile

pngs: $(PNGFILES)

list:
	@echo $(PDFFILES) $(PNGFILES)

%.pdf: %.eps
	$(EPS2PDF) $< --outfile $@.tmp.pdf
	gs -dCompatibilityLevel=1.4 -dPDFSETTINGS=/screen -dCompressFonts=true -dSubsetFonts=true -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sOutputFile=$@ -c ".setpdfwrite <</NeverEmbed [ ]>> setdistillerparams" -f $@.tmp.pdf
	rm $@.tmp.pdf

%.png: %.eps
	$(EPS2PNG) $< -background white -alpha remove -alpha off -rotate 90 $@

%.eps: %.plot %.csv boilerplate* Makefile
	$(GNUPLOT) -e "set terminal post monochrome; set output \"$@\"" $<

clean:
	@rm -f $(PDFFILES)


==> results/tao-graph-3/Makefile <==
FIGS = end_to_end

GNUPLOT := gnuplot
EPS2PDF := epstopdf
EPS2PNG := convert
PDFFILES = $(FIGS:=.pdf)
PNGFILES = $(FIGS:=.png)

all: $(PDFFILES) Makefile

pngs: $(PNGFILES)

list:
	@echo $(PDFFILES) $(PNGFILES)

%.pdf: %.eps
	$(EPS2PDF) $< --outfile $@.tmp.pdf
	gs -dCompatibilityLevel=1.4 -dPDFSETTINGS=/screen -dCompressFonts=true -dSubsetFonts=true -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sOutputFile=$@ -c ".setpdfwrite <</NeverEmbed [ ]>> setdistillerparams" -f $@.tmp.pdf
	rm $@.tmp.pdf

%.png: %.eps
	$(EPS2PNG) $< -background white -alpha remove -alpha off -rotate 90 $@

%.eps: %.plot %.csv boilerplate* Makefile
	$(GNUPLOT) -e "set terminal post monochrome; set output \"$@\"" $<

clean:
	@rm -f $(PDFFILES)


==> results/tao-graph-4-2/Makefile <==
FIGS = dpf sage fcfs

GNUPLOT := gnuplot
EPS2PDF := epstopdf
EPS2PNG := convert
PDFFILES = $(FIGS:=.pdf)
PNGFILES = $(FIGS:=.png)

all: $(PDFFILES) Makefile

pngs: $(PNGFILES)

list:
	@echo $(PDFFILES) $(PNGFILES)

%.pdf: %.eps
	$(EPS2PDF) $< --outfile $@.tmp.pdf
	gs -dCompatibilityLevel=1.4 -dPDFSETTINGS=/screen -dCompressFonts=true -dSubsetFonts=true -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sOutputFile=$@ -c ".setpdfwrite <</NeverEmbed [ ]>> setdistillerparams" -f $@.tmp.pdf
	rm $@.tmp.pdf

%.png: %.eps
	$(EPS2PNG) $< -background white -alpha remove -alpha off -rotate 90 $@

%.eps: %.plot %.csv boilerplate* Makefile
	$(GNUPLOT) -e "set terminal post monochrome; set output \"$@\"" $<

clean:
	@rm -f $(PDFFILES)


==> results/tao-graph-4/Makefile <==
FIGS = dpf sage fcfs

GNUPLOT := gnuplot
EPS2PDF := epstopdf
EPS2PNG := convert
PDFFILES = $(FIGS:=.pdf)
PNGFILES = $(FIGS:=.png)

all: $(PDFFILES) Makefile

pngs: $(PNGFILES)

list:
	@echo $(PDFFILES) $(PNGFILES)

%.pdf: %.eps
	$(EPS2PDF) $< --outfile $@.tmp.pdf
	gs -dCompatibilityLevel=1.4 -dPDFSETTINGS=/screen -dCompressFonts=true -dSubsetFonts=true -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sOutputFile=$@ -c ".setpdfwrite <</NeverEmbed [ ]>> setdistillerparams" -f $@.tmp.pdf
	rm $@.tmp.pdf

%.png: %.eps
	$(EPS2PNG) $< -background white -alpha remove -alpha off -rotate 90 $@

%.eps: %.plot %.csv boilerplate* Makefile
	$(GNUPLOT) -e "set terminal post monochrome; set output \"$@\"" $<

clean:
	@rm -f $(PDFFILES)


==> results/tao-graph-5/Makefile <==
FIGS = end_to_end

GNUPLOT := gnuplot
EPS2PDF := epstopdf
EPS2PNG := convert
PDFFILES = $(FIGS:=.pdf)
PNGFILES = $(FIGS:=.png)

all: $(PDFFILES) Makefile

pngs: $(PNGFILES)

list:
	@echo $(PDFFILES) $(PNGFILES)

%.pdf: %.eps
	$(EPS2PDF) $< --outfile $@.tmp.pdf
	gs -dCompatibilityLevel=1.4 -dPDFSETTINGS=/screen -dCompressFonts=true -dSubsetFonts=true -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sOutputFile=$@ -c ".setpdfwrite <</NeverEmbed [ ]>> setdistillerparams" -f $@.tmp.pdf
	rm $@.tmp.pdf

%.png: %.eps
	$(EPS2PNG) $< -background white -alpha remove -alpha off -rotate 90 $@

%.eps: %.plot %.csv boilerplate* Makefile
	$(GNUPLOT) -e "set terminal post monochrome; set output \"$@\"" $<

clean:
	@rm -f $(PDFFILES)


==> results/tao-graph-6/Makefile <==
FIGS = dpf

GNUPLOT := gnuplot
EPS2PDF := epstopdf
EPS2PNG := convert
PDFFILES = $(FIGS:=.pdf)
PNGFILES = $(FIGS:=.png)

all: $(PDFFILES) Makefile

pngs: $(PNGFILES)

list:
	@echo $(PDFFILES) $(PNGFILES)

%.pdf: %.eps
	$(EPS2PDF) $< --outfile $@.tmp.pdf
	gs -dCompatibilityLevel=1.4 -dPDFSETTINGS=/screen -dCompressFonts=true -dSubsetFonts=true -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sOutputFile=$@ -c ".setpdfwrite <</NeverEmbed [ ]>> setdistillerparams" -f $@.tmp.pdf
	rm $@.tmp.pdf

%.png: %.eps
	$(EPS2PNG) $< -background white -alpha remove -alpha off -rotate 90 $@

%.eps: %.plot %.csv boilerplate* Makefile
	$(GNUPLOT) -e "set terminal post monochrome; set output \"$@\"" $<

clean:
	@rm -f $(PDFFILES)


==> results/tao-graph-7/Makefile <==
FIGS = end_to_end

GNUPLOT := gnuplot
EPS2PDF := epstopdf
EPS2PNG := convert
PDFFILES = $(FIGS:=.pdf)
PNGFILES = $(FIGS:=.png)

all: $(PDFFILES) Makefile

pngs: $(PNGFILES)

list:
	@echo $(PDFFILES) $(PNGFILES)

%.pdf: %.eps
	$(EPS2PDF) $< --outfile $@.tmp.pdf
	gs -dCompatibilityLevel=1.4 -dPDFSETTINGS=/screen -dCompressFonts=true -dSubsetFonts=true -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sOutputFile=$@ -c ".setpdfwrite <</NeverEmbed [ ]>> setdistillerparams" -f $@.tmp.pdf
	rm $@.tmp.pdf

%.png: %.eps
	$(EPS2PNG) $< -background white -alpha remove -alpha off -rotate 90 $@

%.eps: %.plot %.csv boilerplate* Makefile
	$(GNUPLOT) -e "set terminal post monochrome; set output \"$@\"" $<

clean:
	@rm -f $(PDFFILES)


==> results/tao-graph-test/Makefile <==
FIGS = end--to__end_t end_to_end_cp

GNUPLOT := gnuplot
EPS2PDF := epstopdf
EPS2PNG := convert
PDFFILES = $(FIGS:=.pdf)
PNGFILES = $(FIGS:=.png)

all: $(PDFFILES) Makefile

pngs: $(PNGFILES)

list:
	@echo $(PDFFILES) $(PNGFILES)

%.pdf: %.eps
	$(EPS2PDF) $< --outfile $@.tmp.pdf
	gs -dCompatibilityLevel=1.4 -dPDFSETTINGS=/screen -dCompressFonts=true -dSubsetFonts=true -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sOutputFile=$@ -c ".setpdfwrite <</NeverEmbed [ ]>> setdistillerparams" -f $@.tmp.pdf
	rm $@.tmp.pdf

%.png: %.eps
	$(EPS2PNG) $< -background white -alpha remove -alpha off -rotate 90 $@

%.eps: %.plot %.csv boilerplate* Makefile
	$(GNUPLOT) -e "set terminal post monochrome; set output \"$@\"" $<

clean:
	@rm -f $(PDFFILES)


==> sections/applications/admission-control.tex <==
% Section: Applications: Admission Control


==> sections/applications/overview.tex <==
Things that become easier to do now that the privacy resource is integrated into Kub.

==> sections/applications/privacy-resource-visualization.tex <==
% Section: Applications: Privacy Resource Monitoring with Grafana

==> sections/applications/workload-specific-scheduling.tex <==
% Section: Applications: Workload Specific Scheduling

Assume things about the workloads, design a scheduler that works better than the default from previous section for these workloads:

- Recurrent workloads

- Exponential data decay

Potentially a separate section of its own, not just an subsection in Applications.

==> sections/evaluation/methodology.tex <==
% Methodology

\subsubsection{Microbenchmarks}
\label{sec:evaluation:methodology:microbenchmarks}

\subsubsection{Macrobenchmarks}
\label{sec:evaluation:methodology:macrobenchmarks}

\subsubsection{Metrics and Baselines}
\label{sec:evaluation:methodology:metrics-baselines}


==> sections/evaluation/performance-profiling.tex <==
% Evaluation:Performance Profiling

\xxx{TODO(Mingen) ideally also by Friday, Dec 4 (since it seems like you have the data already?)}
A single paragraph needed here with some basic numbers for the various \sysname operations: unlock (reserve as Mingen call it), allocate (once the scheduler decides to allocate, how much time does it take to actually do it), consume, and maybe release.
This is here for perfunctory reasons, so I don't think we should include any graphs or complex explanations.
Say that these ops scale linearly with the number of blocks, because you need to do a 2PC sort of thing, and then give average numbers for one block for each operation.  If all of these operations' runtimes are about the same for fixed number of blocks, then we can just say so and give the results for one only.
